Top-down and bottom-up excursions beyond the Standard Model: The example of left-right symmetries in supersymmetry

In this Ph.D thesis three main projects are presented. In the first one the phenomenology associated with the neutralinos and charginos sector of the left-right symmetric supersymmetric model is explored. After a detailed motivation of the study and construction of such models, it is shown that these models can be easily discovered in multi-leptonic final states as they lead to signatures very different from those induced by the Standard Model or its supersymmetric version. In the second project, we concentrate on the phenomenology associated with doubly-charged particles. Starting from the hypothesis that such a particle is discovered at the LHC, we build several effective field theories depending on both the representation under SU(2)_L to which they belong the particle and their spin and perform a Monte Carlo analysis highlighting some key observables that would help to determine their quantum numbers. Another part of my thesis, complementary to the phenomenology work, has consisted in developping computer programs that might be helpful for phenomenological studies. Working in the framework of the Mathematica package FeynRules, I took part in the development of a routine able to extract automatically the analytical expressions of the renormalization group equations at the two-loop level for any renormalizable supersymmetric model. I have also been involved in the development of another module of FeynRules able to extract automatically the analytical expressions for the mass matrices associated to any model implemented in FeynRules and to export these equations in the form of a C++ source code able to diagonalize the matrices and store the mixing matrices as well as the spectrum in an SLHA-compliant file.

==> mcite/Makefile <==
# Makefile -- install mcite
# Copyright (C) 1994 Thorsten.Ohl@Physik.TH-Darmstadt.de
#
# Mcite is free software; you can redistribute it and/or modify it
# under the terms of the GNU General Public License as published by 
# the Free Software Foundation; either version 2, or (at your option)
# any later version.
#
# Mcite is distributed in the hope that it will be useful, but
# WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the 
# GNU General Public License for more details.
#
# You should have received a copy of the GNU General Public License
# along with this program; if not, write to the Free Software
# Foundation, Inc., 675 Mass Ave, Cambridge, MA 02139, USA.
#
# $Header: /home/sources/ohl/tex/thotex/mcite/Makefile,v 1.4 1996/01/01 23:52:29 ohl Exp $
#
########################################################################

# The name of the game
PROJECT = mcite

# foo.sty, foo.cls, or foo.tex ???
STY = sty

VERSION = 0
RELEASE = 4
STATUS  = beta

########################################################################

# Directories
prefix = $(HOME)
texdir = $(prefix)/tex/inputs
mfdir = $(prefix)/mf/inputs
docdir = $(texdir)/doc

# Commands
INSTALL_DATA = install -c -m 644
# INSTALL_DATA = cp

# This has to be the new LaTeX
LATEX = latex
MAKEINDEX = makeindex
BIBTEX = bibtex

########################################################################
# No user serviceable parts below:
########################################################################

all: $(PROJECT).$(STY) $(PROJECT).drv

dvi: $(PROJECT).dvi

install: all
	$(INSTALL_DATA) $(PROJECT).$(STY) $(texdir)

install.doc: all
	$(INSTALL_DATA) $(PROJECT).dtx $(PROJECT).drv $(docdir)

uninstall:
	rm -f $(texdir)/$(PROJECT).$(STY)

uninstall.doc:
	rm -f $(docdir)/$(PROJECT).dtx
	rm -f $(docdir)/$(PROJECT).drv

$(PROJECT).$(STY): $(PROJECT).dtx $(PROJECT).ins
	$(LATEX) $(PROJECT).ins

$(PROJECT).drv htex.drv hyperbasics.tex: $(PROJECT).$(STY)

$(PROJECT).dvi: $(PROJECT).dtx $(PROJECT).drv \
		$(PROJECT).$(STY) hyperbasics.tex
	-$(LATEX) $(PROJECT).drv
	$(BIBTEX) $(PROJECT)
	$(MAKEINDEX) -s gind.ist -o $(PROJECT).ind $(PROJECT).idx
	$(MAKEINDEX) -s gglo.ist -o $(PROJECT).gls $(PROJECT).glo
	$(LATEX) $(PROJECT).drv
	while grep 'Rerun to get cross-references right\.' $(PROJECT).log; \
	do \
	  $(LATEX) $(PROJECT).drv; \
	done

clean:
	rm -f *.log *.ps *.dv[ij] *.aux *.toc *.lof *.lot \
	      *.[bi]lg *.glo *.gls *.idx *.ind *.bbl \
	      *.hrf '#*#' *~ .*~

realclean: clean
	rm -f $(PROJECT).$(STY) $(PROJECT).drv

distclean: realclean

########################################################################
# Maintenance:

DISTFILES = /usr/local/etc/COPYING README Makefile \
		$(PROJECT).dtx $(PROJECT).ins $(PROJECT).bib

distdir = $(PROJECT)-$(VERSION).$(RELEASE)$(STATUS)
CVSTAG = $(PROJECT)_$(VERSION)_$(RELEASE)$(STATUS)
M = 

commit:
	@if test -n "$(M)"; then \
	  echo "cvs commit -m '$(M)'"; cvs commit -m '$(M)'; \
	  echo "cvs tag $(CVSTAG)"; cvs tag $(CVSTAG); \
	  echo "cvs tag -b $(CVSTAG)_"; cvs tag -b $(CVSTAG)_; \
	else \
	  echo "usage: make commit M='<message>'" 1>&2; \
	fi

dist: $(distdir).tar.gz
snap: $(PROJECT)-current.tar.gz

$(distdir).tar.gz:
	rm -fr $(distdir) $(distdir).tmp
	cvs export -r $(CVSTAG) -d $(distdir).tmp $(PROJECT)
	mkdir $(distdir)
	(cd ./$(distdir).tmp; cp $(DISTFILES) ../$(distdir))
	tar cf - $(distdir) | gzip > $@
	rm -fr $(distdir) $(distdir).tmp

$(PROJECT)-current.tar.gz: $(DISTFILES)
	rm -fr $(PROJECT)-current
	mkdir $(PROJECT)-current
	cp $(DISTFILES) $(PROJECT)-current
	tar cf - $(PROJECT)-current | gzip > $@
	rm -fr $(PROJECT)-current

########################################################################
# Local Variables:
# mode:text
# End:

